An Internal Logic of Virtual Double Categories

We present a type theory called fibrational virtual double type theory (FVDblTT) designed specifically for formal category theory, which is a succinct reformulation of New and Licata's Virtual Equipment Type Theory (VETT). FVDblTT formalizes reasoning on isomorphisms that are commonly employed in category theory. Virtual double categories are one of the most successful frameworks for developing formal category theory, and FVDblTT has them as a theoretical foundation. We validate its worth as an internal language of virtual double categories by providing a syntax-semantics duality between virtual double categories and specifications in FVDblTT as a biadjunction.

==> newsubfiles/constructor/others_thesis.tex <==
\myparagraph{Composition protype $\odot$ for the composites}
The composition protype is the protype that represents the composition of 
paths of loose arrows just of length 2 in virtual double categories
\Cref{def:composite}.

In order to gain access to the composition of paths of positive length in the type theory,
we introduce the \emph{composition protype} $\odot$ to \ac{FVDblTT}.
The formation rule for the composition protype is the following:
\[
    \inferrule*
    {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\ \textsf{protype} \\ 
    \syn{x}:\syn{J}\smcl\syn{y}:\syn{K}\vdash \syn{\beta}(\syn{x}\smcl\syn{y})\ \textsf{protype}}
    {\syn{w}:\syn{I}\smcl\syn{y}:\syn{K}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\odot_{\syn{x}: \syn{J}}\syn{\beta}(\syn{x}\smcl\syn{y})\ \textsf{protype}}
\]
This comes equipped with the introduction rule:
\[
    \inferrule*
    {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\ \textsf{protype} \\
            \syn{x}:\syn{J}\smcl\syn{y}:\syn{K}\vdash \syn{\beta}(\syn{x}\smcl\syn{y})\ \textsf{protype} }
            {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\smcl\syn{y}:\syn{K}\mid \syn{a}:\syn{\alpha}(\syn{w}\smcl\syn{x})\smcl\syn{b}:\syn{\beta}(\syn{x}\smcl\syn{y})\vdash
            \syn{a}\odot\syn{b}:\syn{\alpha}(\syn{w}\smcl\syn{x})\odot_{\syn{x}:\syn{J}}\syn{\beta}(\syn{x}\smcl\syn{y})}
\]
For the detailed rules of the composition protype, see \Cref{sec:composition-protype}.
Plus, we need the compatibility rules for the composition protype and the product types
as we did for the path protype, see \Cref{sec:compo-protype-meets-product-type}.

If we load the path protype $\ides$ and the composite protype $\odot$ to \ac{FVDblTT},
procontexts can be equivalently expressed by a single protype.
In this sense, such a type theory can be seen as an internal language of double categories.
This is supported by the fact that a \ac{VDC} is equivalent to one arising from a double category 
if and only if it has composites of all paths of loose arrows, including units
\cite[Theorem 5.2]{cruttwellUnifiedFrameworkGeneralized2010}.

The semantics of the composition protypes $\odot$ is given by the composites in \acp{VDC} if they have ones of sequences
of length 2 in an appropriate way.
For example, in the \ac{VDC} $\Prof$, the composite of paths of length 2 is the composite of profunctors,
given by the coend $\int$.
In the \ac{VDC} $\Rel{}$, the composites of paths of length 2 are the composites of relations,
given by the existential quantification $\exists$.
\[
    \begin{aligned}
        \sem{\syn{\alpha}(\syn{w}\smcl\syn{x})\odot_{\syn{x}:\syn{J}}\syn{\beta}(\syn{x}\smcl\syn{y})}&=
        \int^{X\in\sem{\syn{J}}}\sem{\syn{\alpha}}(-,X)\times\sem{\syn{\beta}}(X,\bullet)\colon\sem{\syn{I}}\sto\sem{\syn{K}}\  \text{in}\ \Prof{}\\
        \sem{\syn{\alpha}(\syn{w}\smcl\syn{x})\odot_{\syn{x}:\syn{J}}\syn{\beta}(\syn{x}\smcl\syn{y})}&=
        \left\{\,(w,y)\mid\exists x\in\sem{\syn{J}}.\sem{\syn{\alpha}}(w,x)\land\sem{\syn{\beta}}(x,y)\,\right\}\colon\sem{\syn{I}}\sto\sem{\syn{K}}\ \text{in}\ \Rel{}
    \end{aligned}
\]

\myparagraph{Filler protype $\triangleright,\triangleleft$ for the closed structure}
Having obtained the ability to express a particular kind of coends in formal category theory,
and existential quantification in predicate logic,
we would like to introduce the protypes for ends and universal quantification in the type theory.
First of all, we recall the definition of the right extension and the right lift \cite{riehlElementsCategoryTheory2022,arkorFormalTheoryRelative2024} in a \ac{VDC},
which are straightforward generalizations of the right extension and the right lift in a bicategory.

\begin{definition}
    A \emph{right extension} of a loose arrow $\beta\colon I\sto K$ along a loose arrow $\alpha\colon I\sto J$ 
    is a loose arrow $\alpha\triangleright\beta\colon J\sto K$ equipped with a cell
    \[
        \begin{tikzcd}[virtual, column sep=small]
            I
            \sar[r, "\alpha"]
            \ar[d, equal]
            \ar[rrd, phantom, "\varpi_{\alpha,\beta}"]
            &
            J
            \sar[r, "\alpha\triangleright\beta"]
            &
            K
            \ar[d, equal]
            \\
            I
            \sar[rr, "\beta"']
            &&
            K
        \end{tikzcd}
    \]
    with the following universal property.
    Given any cell $\nu$ on the left below where $\ol\gamma$ is an arbitrary sequence of loose arrows,
    it uniquely factors through the cell $\varpi_{\alpha,\beta}$ as on the right below.
    \[
        \begin{tikzcd}[virtual, column sep=small]
            I
            \sar[r, "\alpha"]
            \ar[d, equal]
            \ar[phantom,rrrd, "\nu"]
            &
            J
            \sard[rr, "\ol\gamma"]
            &&
            K 
            \ar[d, equal]
            \\
            I
            \sar[rrr, "\beta"']
            &&&
            K
        \end{tikzcd}
        =
        \begin{tikzcd}[virtual, column sep=small]
            I
            \sar[r, "\alpha"]
            \ar[d, equal]
            \ar[dr, phantom, description, "{\rotatebox{90}{=}}"]
            &
            J
            \ar[d, equal]
            \ar[drr,phantom, "\wt{\nu}"]
            \sard[rr, "\ol\gamma"]
            &&
            K
            \ar[d, equal]
            \\
            I
            \sar[r, "\alpha"']
            \ar[d, equal]
            \ar[phantom,rrrd, "\varpi_{\alpha,\beta}", yshift=-1ex]
            &
            J
            \sar[rr, "\alpha\triangleright\beta"']
            &
            &
            K
            \ar[d, equal]
            \\
            I
            \sar[rrr, "\beta"']
            &&&
            K
        \end{tikzcd}
    \]

    A \emph{right lift} of a protype $\beta\colon I\sto K$ along a protype $\alpha\colon J\sto K$
    is a protype $\beta\triangleleft\alpha\colon I\sto J$ equipped with a cell
    \[
        \begin{tikzcd}[virtual, column sep=small]
            I
            \sar[r, "{\beta\triangleleft\alpha}"]
            \ar[d, equal]
            \ar[rrd, phantom, "\varpi'_{\alpha,\beta}"]
            &
            J
            \sar[r, "\alpha"]
            &
            K
            \ar[d, equal]
            \\
            I
            \sar[rr, "\beta"']
            &&
            K
        \end{tikzcd}
    \]
    with the following universal property.
    Given any cell $\nu$ on the left below where $\ol\gamma$ is an arbitrary sequence of loose arrows,
    it uniquely factors through the cell $\varpi'_{\alpha,\beta}$ as on the right below.
    \[
        \begin{tikzcd}[virtual, column sep=small]
            I
            \sard[rr, "\ol\gamma"]
            \ar[d, equal]
            \ar[phantom,rrrd, "\nu"]
            &&
            J
            \sar[r, "\alpha"]
            &
            K 
            \ar[d, equal]
            \\
            I
            \sar[rrr, "\beta"']
            &&&
            K
        \end{tikzcd}
        =
        \begin{tikzcd}[virtual, column sep=small]
            I
            \sard[rr, "\ol\gamma"]
            \ar[d, equal]
            \ar[drr, phantom, description, "\wt\nu"]
            &&
            J
            \ar[d, equal]
            \ar[dr,phantom, "{\rotatebox{90}{=}}"]
            \sar[r, "\alpha"]
            &
            K
            \ar[d, equal]
            \\
            I
            \sar[rr, "{\beta\triangleleft\alpha}"']
            \ar[d, equal]
            \ar[phantom,rrrd, "\varpi'_{\alpha,\beta}", yshift=-1ex]
            &&
            J
            \sar[r, "\alpha"']
            &
            K
            \ar[d, equal]
            \\
            I
            \sar[rrr, "\beta"']
            &&&
            K
        \end{tikzcd}
    \]
\end{definition}
With this notion, one can handle the concept of weighted limits and colimits internally in virtual double categories.
We now introduce the \emph{filler protypes} $\triangleright$ and $\triangleleft$ to \ac{FVDblTT} 
to express the right extension and the right lift in the type theory.
The formation rule for the \emph{right extension protype} is the following:
\[
    \inferrule*
    {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\ \textsf{protype} \\
    \syn{w}:\syn{I}\smcl\syn{y}:\syn{K}\vdash \syn{\beta}(\syn{w}\smcl\syn{y})\ \textsf{protype}}
    {\syn{x}:\syn{J}\smcl\syn{y}:\syn{K}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\triangleright_{\syn{w}:\syn{I}}\syn{\beta}(\syn{w}\smcl\syn{y})\ \textsf{protype}}
\]
The constructor for the right extension protype is given in the elimination rule 
since the orientation of the universal property of the right extension is 
opposite to that of the composition protype and the path protype.
\[
    \inferrule*
    {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\ \textsf{protype} \\
    \syn{w}:\syn{I}\smcl\syn{y}:\syn{K}\vdash \syn{\beta}(\syn{w}\smcl\syn{y})\ \textsf{protype}}
    {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\smcl\syn{y}:\syn{K}\mid \syn{a}:\syn{\alpha}(\syn{w}\smcl\syn{x})\smcl \syn{e}:\syn{\alpha}(\syn{w}\smcl\syn{x})\triangleright_{\syn{w}:\syn{I}}\syn{\beta}(\syn{w}\smcl\syn{y})\vdash \syn{a}\rbl\syn{e}:\syn{\beta}(\syn{w}\smcl\syn{y})}
\]

The semantics of the right extension protype $\triangleright$ is given by the right extension in \acp{VDC}.
The constructor $\rbl$ is interpreted using the cell $\varpi_{\sem{\syn{\alpha}},\sem{\syn{\beta}}}$ above.
To illustrate the semantics of the right extension protype,
we give the interpretations of the right extension protype in the \acp{VDC} $\Prof{}$ and $\Rel{}$.
\[
    \begin{aligned}
        \sem{\syn{\alpha}(\syn{w}\smcl\syn{x})\triangleright_{\syn{w}:\syn{I}}\syn{\beta}(\syn{w}\smcl\syn{y})}&=
        \int_{W\in\sem{\syn{I}}}\left[\sem{\syn{\alpha}}(W,-),\sem{\syn{\beta}}(W,\bullet)\right]\colon\sem{\syn{J}}\sto\sem{\syn{K}}\  \text{in}\ \Prof{}\\
        \sem{\syn{\alpha}(\syn{w}\smcl\syn{x})\triangleright_{\syn{w}:\syn{I}}\syn{\beta}(\syn{w}\smcl\syn{y})}&=
        \left\{\,(x,y)\mid\forall w\in\sem{\syn{I}}.\left(\sem{\syn{\alpha}}(w,x)\Rightarrow\sem{\syn{\beta}}(w,y)\right)\,\right\}\colon\sem{\syn{J}}\sto\sem{\syn{K}}\ \text{in}\ \Rel{}
    \end{aligned}
\]
Here, $[X,Y]$ is the function set from $X$ to $Y$.

\myparagraph{Comprehension type $\cmpr{\mhyphen}$ for the tabulators}
The last one is not a protype but a type constructor.
First, we note that the definition of tabulators \Cref{def:tabulators}
is directly generalizable to virtual double categories,
where we interpret the triangle cells in the definition as cells with nullary inputs.

Corresponding to the tabulators in virtual double categories,
we introduce the \emph{comprehension type} $\cmpr{\mhyphen}$ to \ac{FVDblTT}.
The formation rule for the comprehension type is the following:
\[
    \inferrule*
    {\syn{x}:\syn{I}\smcl\syn{y}:\syn{J}\vdash \syn{\alpha}\ \textsf{protype}}
    {\cmpr{\syn{\alpha}} \ \textsf{type}}
\]
This comes equipped with the constructor
\[
    \inferrule*
    {\syn{x}:\syn{I}\smcl\syn{y}:\syn{J}\vdash \syn{\alpha}\ \textsf{protype}}
    {\syn{w}:\cmpr{\syn{\alpha}}\vdash \syn{l}(\syn{w}):\syn{I}\\
    \syn{w}:\cmpr{\syn{\alpha}}\vdash \syn{r}(\syn{w}):\syn{J}\\
    \syn{w}:\cmpr{\syn{\alpha}}\mid \vdash \tabb_{\cmpr{\syn{\alpha}}}(\syn{w}):\syn{\alpha}[\syn{l}(\syn{w})/\syn{x}\smcl\syn{r}(\syn{w})/\syn{y}]}
\]

The comprehension type $\cmpr{\mhyphen}$ is interpreted as the tabulators in the \acp{VDC}.
In the \ac{VDC} $\Prof$,
the tabulator of a profunctor $P\colon\one{C}\sto\one{D}$ is given 
by \emph{two-sided Grothendieck construction},
which results in \emph{a two-sided discrete fibration} from $\one{C}$ to $\one{D}$.
A frequently used example of this construction is
the comma category for a pair of functors $F\colon\one{C}\to\one{E}$ and $G\colon\one{D}\to\one{E}$
as the tabulator of the profunctor $\one{E}(F(-),G(-))$,
see \cite{loregianCategoricalNotionsFibration2020} for more details.
The \ac{VDC} $\Rel{}$ has the tabulators
if we ground the double category to an axiomatic system of set theory with the comprehension axiom,
as the tabulator of a relation $R\colon A\sto B$ is given by the set of all the pairs $(a,b)$ such that $R(a,b)$ holds.

In the presence of the unit protype $\ide{}$, 
we should add some rules concerning the compatibility between the comprehension type and the path protype.
This is because, in many examples of double categories, the tabulators have not only the universal property
as in \Cref{def:tabulators} but also respect the units,
although the original universal property of the tabulators is enough to detect the tabulators in a double category.
This issue is thoroughly discussed in \cite{grandisLimitsDoubleCategories1999}.
Here, we give a slightly generalized version of the tabulators in virtual double categories with units.
\begin{definition}[2-dimensional universal property of tabulators]
    In a virtual double category with units, a \emph{unital tabulator} $\{\alpha\}$ of a loose arrow $\alpha\colon I\sto J$
    is a tabulator of $\alpha$ in the sense of \Cref{def:tabulators}, which also satisfies the following universal property.
    Suppose we are given any pair of cones $(X,h,k,\nu)$ and $(X',h',k',\nu')$ over $\alpha$
    and a pair of cells $\varsigma,\vartheta$ such that the following equality holds.
    \[
        \begin{tikzcd}[virtual]
            X
            \sard[r, "\ol\gamma"]
            \ar[rd, phantom, "\varsigma"]
            \ar[d, "h"']
            &
            X'
            \ar[d, "h'"']
            \ar[dr, phantom, "\nu'", yshift=-1ex, xshift=-2ex]
            \ar[dr,"k'"]
            \\
            I
            \sar[r, "U_I"']
            \ar[d, equal]
            \ar[drr, phantom, "{\rotatebox{90}{$\cong$}}"]
            &
            I
            \sar[r, "\alpha"']
            &
            J
            \ar[d, equal]
            \\
            I 
            \sar[rr, "\alpha"']
            &&
            J
        \end{tikzcd}
        =
        \begin{tikzcd}[virtual]
            &
            X
            \ar[dl, "h"']
            \ar[d, "k"]
            \sard[r, "\ol\gamma"]
            \ar[dr, phantom, "\vartheta"]
            \ar[dl, phantom, "\nu", yshift=-1ex, xshift=1ex]
            &
            X'
            \ar[d, "k'"]
            \\
            I
            \sar[r, "\alpha"']
            \ar[d, equal]
            \ar[rrd, phantom, "{\rotatebox{90}{$\cong$}}"]
            &
            J
            \sar[r, "U_J"']
            &
            J
            \ar[d, equal]
            \\
            I
            \sar[rr, "\alpha"']
            &&
            J
        \end{tikzcd}
    \]
    Then, there exists a unique cell $\varrho$ for which the following equalities hold.
    \[
        \begin{tikzcd}[virtual]
            X
            \sard[r, "\ol\gamma"]
            \ar[d, "t_{\nu}"']
            \ar[rd, phantom, "\varrho"]
            &
            X'
            \ar[d, "t_{\nu'}"]
            \\
            \{\alpha\}
            \sar[r, "U_{\{\alpha\}}"']
            \ar[d, "\ell_{\alpha}"']
            \ar[dr, phantom, "U_{\ell_\alpha}"description, yshift=-1ex]
            &
            \{\alpha\}
            \ar[d, "\ell_{\alpha}"]
            \\
            I
            \sar[r, "U_I"']
            &
            I
        \end{tikzcd}
        =
        \begin{tikzcd}[virtual]
            X
            \sard[r, "\ol\gamma"]
            \ar[d, "h"']
            \ar[rd, phantom, "\varsigma"]
            &
            X'
            \ar[d, "h'"]
            \\
            I
            \sar[r, "U_I"']
            &
            I
        \end{tikzcd}
        \quad
        ,
        \quad
        \begin{tikzcd}[virtual]
            X
            \sard[r, "\ol\gamma"]
            \ar[d, "t_{\nu}"']
            \ar[rd, phantom, "\varrho"]
            &
            X'
            \ar[d, "t_{\nu'}"]
            \\
            \{\alpha\}
            \sar[r, "U_{\{\alpha\}}"']
            \ar[d, "r_{\alpha}"']
            \ar[dr, phantom, "U_{r_\alpha}"description, yshift=-1ex]
            &
            \{\alpha\}
            \ar[d, "r_{\alpha}"]
            \\
            J 
            \sar[r, "U_J"']
            &
            J
        \end{tikzcd}
        =
        \begin{tikzcd}[virtual]
            X
            \sard[r, "\ol\gamma"]
            \ar[d, "k"']
            \ar[rd, phantom, "\vartheta"]
            &
            X'
            \ar[d, "k'"]
            \\
            J
            \sar[r, "U_J"']
            &
            J
        \end{tikzcd}
    \]
\end{definition}
This universal property determines what the unit on the apex of the tabulator should be. 
\Cref{sec:comprehension-type-meets-unit-protype} will present the corresponding rules for the comprehension type $\cmpr{\mhyphen}$ in \ac{FVDblTT} with the unit protype $\ides$.

\begin{remark}[Substitution into the additional constructor]
    \label{rem:substitution-into-additional-constructor}
    There are options how we define substitution for the additional constructors.
    For example, we may define the substitution for the composition protype as follows.
    \[
    (\syn{\alpha}\odot_{\syn{y}:\syn{J}}\syn{\beta})[\syn{s}/\syn{x}\smcl\syn{t}/\syn{z}]
    \coloneqq
    \syn{\alpha}[\syn{s}/\syn{x}\smcl\syn{y}/\syn{y}]\odot_{\syn{y}:\syn{J}}\syn{\beta}[\syn{y}/\syn{y}\smcl\syn{t}/\syn{z}] 
    \]
    This seems reasonable for our use in formal category theory,
    but this equality is not always satisfied in a general PL-composable \ac{FVDC}
    unless it is actually a virtual equipment.
    Instead, we may extend the introduction rule for the composition protype 
    so that the substituted composition protypes are directly introduced.
    \[
    \inferrule*
    {\syn{w}:\syn{I}\smcl\syn{x}:\syn{J}\vdash \syn{\alpha}(\syn{w}\smcl\syn{x})\ \textsf{protype} \\
    \syn{x}:\syn{J}\smcl\syn{y}:\syn{K}\vdash \syn{\beta}(\syn{x}\smcl\syn{y})\ \textsf{protype} \\
    \syn{\Gamma}\vdash \syn{s}:\syn{I} \\
    \syn{\Delta}\vdash \syn{t}:\syn{K}}
    {\syn{\Gamma}\smcl\syn{\Delta}\vdash (\syn{\alpha}\odot_{\syn{x}:\syn{J}}\syn{\beta})[\syn{s}/\syn{w}\smcl\syn{t}/\syn{y}]: \textsf{protype}}
    \]
    Then, the substitution for the composition protype is obvious.
    Indeed we take the latter approach for the path protype.

    Therefore, it depends on the purpose of the type theory how we define the substitution for the additional constructors,
    and we do not specify it in this paper because our main focus is the syntax-semantics duality
    for the very basic type theory.
\end{remark}

==> newsubfiles/constructor/predlogic_thesis.tex <==
\myparagraph{Predicate logic.}
\label{sec:arrangement-for-predicate-logic}

When we work with the type theory \ac{FVDblTT} for the purpose of reasoning about predicate logic,
we consider types, terms, protypes, and proterms to represent sets, functions, predicates (or propositions), and proofs, respectively. 
However, the type theory \ac{FVDblTT}, as it is, treats the protypes in a context $\syn{\Gamma}\smcl\syn{\Delta}$ and
those in a context $\syn{\Delta}\smcl\syn{\Gamma}$ as different things.
In this sense, the type theory \ac{FVDblTT} as predicate logic has directionality.
If one wants to develop a logic without a direction,
one can simply add the following rules to the type theory.

    \begin{mathparpagebreakable}
        \inferrule*
        {\syn{\Gamma}\smcl\syn{\Delta}\vdash \syn{\alpha} \ \textsf{protype}}
        {\syn{\Delta}\smcl\syn{\Gamma}\vdash \syn{\alpha}^\circ \ \textsf{protype}}
        \and
        \inferrule*
        {\syn{\Gamma}_0\smcl\cdots\smcl\syn{\Gamma}_m\mid \syn{a}_1:\syn{\alpha}_1\cdots \syn{a}_n:\syn{\alpha}_n
        \vdash \syn{\mu}:\syn{\beta}}
        {\syn{\Gamma}_m\smcl\cdots\smcl\syn{\Gamma}_0\mid \syn{a}_n:\syn{\alpha}_n^\circ\cdots \syn{a}_1:\syn{\alpha}_1^\circ
        \vdash \syn{\mu}^\circ:\syn{\beta}^\circ}
        \and
        \inferrule*
        {\syn{\Gamma}_0\smcl\cdots\smcl\syn{\Gamma}_m\mid \syn{a}_1:\syn{\alpha}_1\cdots \syn{a}_n:\syn{\alpha}_n
        \vdash \syn{\mu}:\syn{\beta}}
        {\syn{\Gamma}_0\smcl\cdots\smcl\syn{\Gamma}_m\mid \syn{a}_1:\syn{\alpha}_1\cdots \syn{a}_n:\syn{\alpha}_n
        \vdash \syn{\mu}^{\circ\circ}\equiv\syn{\mu}:\syn{\beta}}
    \end{mathparpagebreakable}
These rules are the counterparts of the structure of involution in \acp{VDC}.

This perspective is better understood with the $\Bil$-construction in \Cref{chapter:HDas}.
This operation sending a cartesian fibration to a \ac{CFVDC} corresponds to 
translating predicate logic with proofs as an internal logic of cartesian fibrations \Cref{rem:intlang}
in terms of the type theory \ac{FVDblTT}.
More precisely, there is a comparison virtual double functor from the $\Bil$ of the syntactic cartesian fibration 
to the syntactic \ac{VDC} in \Cref{sec:synsemadj}.
This seems to be the 1-cell into the syntactic \ac{VDC} from its 
``cofree Frobenius \ac{CFVDC}'' in the 2-category of \acp{CFVDC},
although we do not have a formal proof of this statement and leave it as a conjecture.

If one also wants to make the type theory \ac{FVDblTT} proof irrelevant,
one can reformulate protype isomorphism judgment as equality judgments of protypes 
and add the rule stating that all the proterms are equal.
It is the counterpart of the flatness \cite{grandisLimitsDoubleCategories1999} or local preorderedness
\cite{hoshinoDoubleCategoriesRelations2023} of \acp{VDC}. 


==> newsubfiles/constructor/tableofconstructorshort.tex <==
This section will specify the type and protype constructors that can be added to \ac{FVDblTT}.
The \acp{VDC} of relations and those of profunctors have many structures in common.
We would like to introduce the inductive types and protypes corresponding to the common structures in these kinds of \acp{VDC},
as summarized in \Cref{table:commonconst}.
We will only address the units in this paper and leave the other constructors to \Cref{appendix:moreconstructors}.

\begin{table}[h] 
    \rowcolors{2}{gray!25}{white}
    \begin{tabular}{|c||c|c||c|}
        \hline
        \rowcolor{gray!50}
        \textbf{Structures} & \textbf{Formal category theory} & \textbf{Predicate logic} & \begin{tabular}{@{}c@{}}\textbf{Constructors}\\ \textbf{in FVDblTT}\end{tabular}\\
        \hline
        \hline
        Units \cite{cruttwellUnifiedFrameworkGeneralized2010} & hom-profuntors $\one{C}(-,\bullet)$ & equality $=$ & path $\ides$ \\
        Composition \cite{cruttwellUnifiedFrameworkGeneralized2010} & composition via coends $\int$ & composition via $\exists$ & composition $\odot$ \\
        Extension \cite{riehlElementsCategoryTheory2022} & profunctor extension $\triangleright$ & contraction via $\forall$ & extension $\triangleright$ \\
        Tabulators \cite{grandisLimitsDoubleCategories1999} & \begin{tabular}{@{}c@{}}two-sided\\ Grothendieck construction\end{tabular} & comprehension $\{\mhyphen\}$ & tabulator $\cmpr{\mhyphen}$ \\
        \hline
    \end{tabular} 
    \caption{The common structures and the corresponding constructors}
    \label{table:commonconst}
\end{table}


==> newsubfiles/constructor/units_thesis.tex <==

\myparagraph{Path protype $\ides$ for the units}
The path protype is the protype that represents the units in a \ac{VDC}.
In a double category, the units are just the identity loose morphisms,
but in a \ac{VDC}, the units are formulated via a universal property \Cref{def:composite,def:composable}.

The formation rule for the \emph{path protype} is on the left below, and it comes equipped with the introduction rule on the right below: 
    
    \begin{mathparpagebreakable}
    \inferrule*[right=$\ides$-Form]
    {\syn{I}\ \textsf{type}\\
    \syn{\Gamma}\vdash \syn{s}:\syn{I}\\
    \syn{\Delta}\vdash \syn{t}:\syn{I}}
    {\syn{\Gamma}\smcl\syn{\Delta}\vdash \syn{s}\ide{\syn{I}}\syn{t}\ \textsf{protype}}
    \and
    \inferrule*
    {\syn{I}\ \textsf{type}}
    {\syn{x}:\syn{I}\mid \quad \vdash \refl_{\syn{I}}(\syn{x}): \syn{x}\ide{\syn{I}}\syn{x}} 
    \end{mathparpagebreakable}
The proterm $\refl$ corresponds to the unit $\eta_I$ in the definition of the units.
To let the path protype encode the units in the \acp{VDC},
we need to add elimination and computation rules as in \Cref{sec:unit-protype}.
The path protypes behave as inductive (pro)types,
and their inductions look very similar to path induction in homotopy type theory,
but with the difference that the path protype is directed.

The semantics of the path protypes $\ides$ are given by the units in any \ac{VDC} with units,
with the proterm constructor $\refl_{\syn{I}}$ interpreted as the cell $\eta_{\sem{\syn{I}}}$.
For instance, in the \acp{VDC} $\PROF$ and $\Rel{}$, the interpretations of the path protypes are given as
the hom profunctors and the equality relations, respectively.
These follow from the fact that the identity loose morphisms in a double category serve as the units when we see it as a \ac{VDC}.

In order to make the path protypes behave well with the product types in \ac{FVDblTT},
we need to add the compatibility rules between the path protypes and the product types
as in \Cref{sec:unit-protype-meets-product-type}.
For instance, when we consider the hom-profunctor on a product category $\one{C}\times\one{D}$,
we expect its components to be isomorphic to the product $\one{C}(C,C')\times\one{D}(D,D')$.
Correspondingly, we would like to add the following rule, which does not follow from other rules \textit{a priori}:

    \begin{mathparpagebreakable}
    \inferrule*
    {\syn{I}\ \textsf{type}\\ \syn{J}\ \textsf{type}}
    {\syn{x}:\syn{I},\syn{y}:\syn{J}\smcl\syn{x}':\syn{I},\syn{y}':\syn{J}
    \vdash \exc_{\ides,\land}:\langle\syn{x},\syn{y}\rangle\ide{\syn{I}\times\syn{J}}\langle\syn{x'},\syn{y'}\rangle
    \ccong \syn{x}\ide{\syn{I}}\syn{x}'\land\syn{y}\ide{\syn{J}}\syn{y'}}.
    \end{mathparpagebreakable}
\Cref{sec:unit-protype-meets-product-type} will give the whole set of rules for the compatibility between the path protypes and the product types. 
The rules we introduce are justified by the fact that 
with them, the syntactic \acp{VDC} we will introduce in \Cref{sec:synsemadj}
become cartesian objects in the 2-category of \acp{FVDC} with units.
See \Cref{prop:cartesianunital} for a detailed explanation from the 2-categorical perspective.


==> newsubfiles/discussion/comparison.tex <==
In this section, we will discuss how \ac{FVDblTT}, in comparison with New and Licata's ``Virtual Equipment Type Theory'' (VETT) \cite{newFormalLogicFormal2023},
stands out with its practicality and 2-categorical accuracy in the semantics.
It is protype isomorphism judgments that achieve the practicality, 
and the 2-categorical accuracy is what we have developed in \Cref{sec:synsemadj}.

The most significant difference resides in protype isomorphism judgments in \ac{FVDblTT}.
The equality of sets in VETT does not incorporate isomorphisms into the equational theory.
VETT proves isomorphisms of sets (profunctors) by constructing mutual inverses meta theoretically but cannot
directly reason about them inside the type theory.
\Ac{FVDblTT} directly handles protype isomorphisms inside the type theory and shows what can be done in a \ac{VDC} as it is,
which simulates reasoning on isomorphisms in category theory.
The difference comes partly from the presentation of profunctors.
Profunctors in VETT look like $\phi:\lambda\alpha;\beta.R(\alpha\smcl\beta)$, and ``$\lambda$'' represents quantification that respects the naturality of $\phi$.
Although this kind of presentation suits how one argues about profunctors in ordinary category theory,
it does not reflect how one formally develops category theory in a \ac{VDC}.
In short, VETT is a formal language for category theory that can treat a wide range of category theories,
while \ac{FVDblTT} is a formal language for formal category theory.

The semantics of VETT are given in a \textit{split fibrational virtual equipment},
where all the restrictions are chosen in a compatible way.
If one considers a complete set of connectives given in this paper such as composition or extensions,
the stage of the semantics requires many choices and compatibility conditions,
which are sometimes complicated to handle.
On the other hand, the semantics of \ac{FVDblTT} is given in a \ac{CFVDC} with no restrictions chosen.
We naively interpret the entities of the type theory,
which is justified by allowing the interpretation to be up to equivalence in the 2-category of \acp{VDC}.
In practice, this enables us to take any \ac{VDC} with additional (non-split) structures that we need to interpret the type theory
without worrying about how they are chosen.
On the theoretical side, a syntax-semantics adjunction is, in general, established concerning 2-dimensional structures
since the interpretation of the type theory is given only up to isomorphism.
The author does not know why the initiality of the syntactic model in VETT does not require
2-dimensional care in \cite{newFormalLogicFormal2023}.
In the context of Martin-L\"of type theory, for example, similar problems called the coherence problems have been studied 
in \cite{curienSubstitutionIsomorphism1993,hofmannInterpretationTypeTheory1995,clairambaultBiequivalenceLocallyCartesian2014}.
This paper is intended to give a 2-categorically accurate semantics of a type theory for formal category theory.
In particular, we pay special attention to how two constructors in the type theory should be interrelated to each other
from the perspective of 2-categories of \acp{VDC} with additional structures, as discussed in \Cref{sec:appendix2},
providing persuasive evidence that the type theory is a beneficial language both
as an internal language for \acp{VDC} and as a language for formal category theory in \acp{VDC}.

It is fair to mention what cannot be done in \ac{FVDblTT} now.
The type theory lacks the meta-level kinds as in VETT,
meaning that we cannot deal with categories or functors using polymorphism in the type theory.
On the other hand, VETT has different type-theoretic entities corresponding to the hierarchy of abstractness.
It has \textit{categories}, \textit{sets}, and meta-level entities called \textit{types}, all with equational theory.
The distinction between categories in VETT and types in \ac{FVDblTT} is that the former has the equational theory as elements
of a meta-level type ``Cat'' while the latter does not.
When we consider the semantics of these type theories, it makes a significant difference that
VETT requires \acp{VDC} indexed by a category with families (VETT judgmental models) as a model,
while \ac{FVDblTT} merely requires a single \ac{VDC}.

\begin{table}[htbp]
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \rowcolors{2}{gray!25}{white}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c||c|c|}
        \toprule
        \rowcolor{gray!50}
        & \textbf{FVDblTT in this paper} & \textbf{VETT in \cite{newFormalLogicFormal2023}} \\
        \midrule
        Type-theoretic entities & types, terms, protypes, proterms & categories, sets, types \\
        \midrule
        Isomorphic reasoning & \checkmark & $\times$ \\
        \midrule
        Semantics & cartesian fibrational \acsp{VDC} & indexed split-fibrational virtual equipments \\
        \midrule
        Syntax-semantics duality & biadjunction & initiality (without 2-dimensional care) \\
        \midrule
        Polymorphism & $\times$ & \checkmark \\
        \bottomrule
    \end{tabular}}
    \caption{Comparison between \ac{FVDblTT} and VETT}
    \label{table:comparison}
\end{table}


==> newsubfiles/prelim/vdcshort.tex <==
In this section, we summarize the terminology and notation that we use in this paper.
We assume that the reader is familiar with the basic concepts of category theory, including 2-categories.
For more details on the definitions concerning virtual double categories, 
see \Cref{sec:previrtual}
or \cite{cruttwellUnifiedFrameworkGeneralized2010,newFormalLogicFormal2023} as references.

\Acp{VDC} are a generalization of ordinary double categories.
In a \ac{VDC}, we have four kinds of data: objects; \emph{tight arrows}, which are depicted vertically;
\emph{loose arrows}, which are depicted horizontally; and \emph{(virtual) cells}, which are depicted as follows:

\[ 
    \begin{tikzcd}[virtual]
        I_0
        \ar[d, "s"']
        \sar[r, "\alpha_1"]
        \ar[rrrd, phantom, "\mu"]
        & I_1
        \sar[r, "\alpha_2"]
        & \cdots
        \sar[r, "\alpha_n"]
        & I_n
        \ar[d, "t"] \\
        J_0
        \sar[rrr, "\beta"']
        & & & J_1
    \end{tikzcd}
    \quad \text{where} \quad
    n \geq 0.
\]
If a cell has the identity arrows as its vertical boundaries, then we call it a \emph{globular cell}
and symbolize it as $\mu\colon \alpha_1\smcl\cdots\smcl\alpha_n\Rightarrow\beta$.
In particular, when $\mu\colon\alpha\Rightarrow\beta$ and $\nu\colon\beta\Rightarrow\alpha$ are globular cells whose inputs
of length 1, and $\mu$ and $\nu$ are mutually inverses to each other with respect to verticle composition, 
then we call $\alpha$ and $\beta$ \emph{isomorphic} and write $\alpha\cong\beta$.

In this paper, we focus on \emph{fibrational virtual double categories}.
Since the terminology around this concept has fluctuated in the literature,
we explicitly define it as follows.
\begin{definition}[{\cite[Definition 7.1]{cruttwellUnifiedFrameworkGeneralized2010}}]
    \label{def:fibrational}
    Let $\dbl{D}$ be a virtual double category. 
    A \emph{restriction} of a loose arrow $\alpha\colon I \sto J$ 
    along a pair of tight arrows $s\colon I' \to I$ and $t\colon J' \to J$ is the loose arrow $\alpha[s\smcl t]\colon I' \sto J'$ 
    equipped with a cell presented on the left below with the universal property
    that any cell $\mu$ of the form on the left below factors uniquely through the cell 
    $\restc$ as on the right below.
    \[
        \begin{tikzcd}[virtual]
            I'
            \ar[d, "s"']
            \sar[r, "{\alpha[s\smcl t]}"]
            \ar[dr, phantom, "\restc"]
            & J'
            \ar[d, "t"] \\
            I
            \sar[r, "\alpha"']
            & J
        \end{tikzcd}
        \quad , \quad
        \begin{tikzcd}[virtual]
            K 
            \ar[d, "u"']
            \sard[r, "\ol\beta"]
            \ar[ddr, phantom, "\mu"]
            & 
            L 
            \ar[d, "v"] \\
            I'
            \ar[d, "s"']
            &
            J'
            \ar[d, "t"] \\
            I
            \sar[r, "\alpha"']
            & J
        \end{tikzcd}
        \quad = \quad
        \begin{tikzcd}[virtual]
            K 
            \ar[d, "u"']
            \sard[r, "\ol\beta"]
            \ar[dr, phantom, "\widehat{\mu}"]
            &
            L
            \ar[d, "v"] \\
            I'
            \ar[d, "s"']
            \sar[r, "{\alpha[s\smcl t]}"']
            \ar[dr, phantom, "{\restc}", yshift=-0.3em]
            & J'
            \ar[d, "t"] \\
            I
            \sar[r, "\alpha"']
            & J
        \end{tikzcd}
    \]
    If the restrictions exist for all triples $(\alpha, s, t)$, then we say that $\dbl{D}$ is a \emph{\ac{FVDC}}.
\end{definition}
We write $\FibVDbl$ for the 2-category of \aclp{FVDC},
virtual double functors preserving restrictions, and vertical transformations between them,
where the last two are defined appropriately.
The representative examples of \acp{FVDC} are the \acp{VDC} of profunctors $\PROF$ and relations $\Rel{}$.

For an arbitrary 2-category, one can define \emph{cartesian objects} therein.
We let $\bi{K}_{\bi{cart}}$ denote the 2-category of cartesian objects in a 2-category $\bi{K}$,
1-cells preserving cartesian structure, and arbitrary 2-cells between them.
What we focus on in this paper is the 2-category $\FibVDbl_{\bi{cart}}$ of \acp{CFVDC}.
A more concrete presentation of this concept is given in \Cref{prop:FibVDblCart}.

==> newsubfiles/typetheory/inddefsemshort.tex <==
We interpret all typing judgments inductively.
For example, the interpretation of the protype $\syn{\alpha}[\syn{S}/\syn{\Gamma}\smcl\syn{T}/\syn{\Delta}]$ is the restriction 
    of the loose arrow $\sem{\syn{\alpha}}:\sem{\syn{\Gamma}}\sto\sem{\syn{\Delta}}$ along the tight arrow
    $\sem{\syn{S}}:\sem{\syn{\Gamma}'}\to \sem{\syn{\Gamma}}$ and $\sem{\syn{T}}:\sem{\syn{\Delta}'}\to \sem{\syn{\Delta}}$.
    \[
        \begin{tikzcd}[column sep=12ex,virtual]
            \sem{\syn{\Gamma}'}
            \sar[r, "{\sem{\syn{\alpha}[\syn{S}/\syn{\Gamma}\smcl\syn{T}/\syn{\Delta}]}}"]
            \ar[d, "\sem{\syn{S}}"']
            \ar[dr,phantom, "\cart" description]
            &
            \sem{\syn{\Delta}'}
            \ar[d, "\sem{\syn{T}}"]
            \\
            \sem{\syn{\Gamma}}
            \sar[r, "\sem{\syn{\alpha}}"']
            &
            \sem{\syn{\Delta}}
        \end{tikzcd}
    \]
The full list of interpretations is given in \Cref{sec:appendix3}.
